Quality meets Diversity: A Model-Agnostic Framework for Computerized Adaptive Testing

Computerized Adaptive Testing (CAT) is emerging as a promising testing application in many scenarios, such as education, game and recruitment, which targets at diagnosing the knowledge mastery levels of examinees on required concepts. It shows the advantage of tailoring a personalized testing procedure for each examinee, which selects questions step by step, depending on her performance. While there are many efforts on developing CAT systems, existing solutions generally follow an inflexible model-specific fashion. That is, they need to observe a specific cognitive model which can estimate examinee's knowledge levels and design the selection strategy according to the model estimation. In this paper, we study a novel model-agnostic CAT problem, where we aim to propose a flexible framework that can adapt to different cognitive models. Meanwhile, this work also figures out CAT solution with addressing the problem of how to generate both high-quality and diverse questions simultaneously, which can give a comprehensive knowledge diagnosis for each examinee. Inspired by Active Learning, we propose a novel framework, namely Model-Agnostic Adaptive Testing (MAAT) for CAT solution, where we design three sophisticated modules including Quality Module, Diversity Module and Importance Module. Extensive experimental results on two real-world datasets clearly demonstrate that our MAAT can support CAT with guaranteeing both quality and diversity perspectives.

==> introduction_old.tex <==
\section{Introduction}
\label{section:intro}

% 第一段，介绍CAT的诞生背景
% assessment -> PPT -> CAT
Diagnosing the ability of the examinees is an important task in many scenarios such as education, vocation and psychology.
A key part in the task is test design, i.e., selecting a set of questions from the question pool for the examinees.
Traditional Pen and Paper Test selects a set of questions at one time beforehand and delivers the identical question set to each examinee.
Although the traditional form is simple and practical, it is believed that the diagnosis will be more accurate if we tailor the tests for examinees,
e.g., provide outstanding examinees with more challenging questions.
This idea gave birth to a promising testing form called \textbf{Computerized Adaptive Testing (CAT)} \cite{wainer2000computerized}.
In order to tailor the test for an examinee, CAT selects a set of questions step by step, depending on the interactive performance of the examinee.
For example, if the recent questions are answered correctly, the next question may be more difficult.
In comparison with traditional tests, CAT has higher accuracy and shorter length, which has been proven in many applications recent years, such as Graduate Management Admission Test (GMAT) \cite{rudner2009implementing} and Graduate Record Examinations (GRE) \cite{mills2000gre}.

% CAT的组成和流程
Specifically, when an examinee (e.g., $e_1$) with unknown ability comes, a typical CAT system starts up an iterative testing procedure as shown in Fig.~\ref{subfig:CATcomponents}.
At step $t$, one question (e.g., $q_t^*)$) is selected from the question pool by a \textit{selection strategy}.
After $e_1$ answers $q_t^*$, a \textit{cognitive diagnosis model} (CDM) (e.g., IRT \cite{embretson2013item}) produces a dynamical ability diagnosis for $e_1$ instantly.
The iteration repeats until a termination condition is met, such as reaching the preset test length.
Our goal is designing the strategy to select appropriate questions so that the diagnosis of the CDM is as accurate as possible.
In this way, the CAT system generates a tailored test sequence for each examinee.
For example, in Fig.~\ref{subfig:CATprocedure}, two examinees, $e_1$ and $e_2$, start with the same question, however perform differently.
Due to the different instant diagnosis caused by their performance, they are provided with tailored questions by the CAT system to make accurate subsequent diagnosis.


\begin{figure}
    \centering
    \subfigure[]{    
        \includegraphics[width=0.45\linewidth]{figures/Fig1a.png}
        \label{subfig:CATcomponents}
    }
    \subfigure[]{    
        \includegraphics[width=0.45\linewidth]{figures/Fig1b.png}
        \label{subfig:CATprocedure}
    }
    \caption{(a) Illustration of a typical CAT system consisting of a question selection strategy and a cognitive diagnosis model, as well as the testing procedure in one step. (b) Two toy examples of CAT procedure. The examinees, $e_1$ and $e_2$, got the same first question at the beginning of the adaptive tests. However, due to their different performance, the following questions are personalized.}
    \label{Fig.1}
    \vspace{-5pt}
\end{figure}


% 概览CAT现有的方法
% 分析CAT目前的不足 -> model-specific
% 提出CAT的理想状态 -> model-agnostic
Over the past years, there have been many studies on CAT, which can be categorized into cognitive diagnosis model development\cite{torre2014cognitively} and selection strategy design\cite{chang2015psychometrics}.
Generally, existing strategies deeply dig into the details of the underlying CDMs and minimize the statistical estimation error of the parameters which have strong interpretation about ability.
For example, \textit{Maximum Fisher Information} \cite{chang2015psychometrics}, an IRT-based selection strategy, greedily selects the question that minimizes the variance of the maximum likelihood estimation of the latent parameter representing the ability level of the examinee in IRT.
Though these works have made remarkable effect, they are all \textbf{model-specific}, i.e., the strategy is only suitable for its own designated CDM.
There are two limitations of being model-specific: (1) the CAT problem becomes nonuniform and hard because we must consider how a specific CDM works in detail when designing the selection strategy; (2) the CAT system becomes inflexible because we must redesign the strategy if we want to replace the CDM.
In principle, the strategy need only care about \textit{what} ability diagnosis the CDM outputs for the examinee, rather than \textit{how} it produces the diagnosis in detail.
Therefore, an ideal CAT framework should be \textbf{model-agnostic}, i.e., the strategy should be independent of the detailed structure and mechanism of the CDM.
In this paper, we propose a redefinition for CAT in which the CDM captures the ability diagnosis with abstract parameters and the details are assumed to be unknown.

% CAT和AL的联系
% 将CAT formulate成AL是可行的
% 需要调整的是goal
Though there has been little previous work on achieving a model-agnostic framework for CAT, we find the similar idea in \textit{Active Learning} (AL), which is a popular framework to alleviate data deficiency in many supervised learning tasks \cite{houlsby2014cold,gal2017deep,cai2019multi}.
Starting with a large set of unlabeled data, AL framework aims to design a strategy to select valuable data step by step for human annotators so that the machine learning model can achieve better performance in the task.
At each step, a batch of data is selected from the unlabeled dataset according to the performance of the model trained on the labeled data.
The general pattern is similar to that of CAT, however with a key difference:
instead of using the model details, most AL strategies only need the output of the model (e.g., label predictions) or the feature of the data (e.g., embedding representations), so that they can be applied to many different models and tasks.
This idea inspires us to provide a model-agnostic framework for CAT.

To this end, we propose a \textbf{M}odel-\textbf{A}gnostic \textbf{A}daptive \textbf{T}esting framework (\textbf{MAAT} for short).
In order to implement a concrete selection strategy, we propose specific goals in MAAT.
The general target of CAT is maximizing the accuracy of the ability diagnosis for examinees.
To achieve that, the questions selected by the strategy should be both high-quality and diverse.
Specifically, the quality of an individual question means how much information we obtain about the examinee when we observe her response to the question.
For example, a question that is either too difficult or too easy is considered to be low-quality since we can hardly know more about the examinee through it.
In contrast, diversity is a collective concept which means how many aspects we cover in a set of questions.
In this paper, we consider diversity at knowledge level.
For example, in a math test, the question set is seen as not diverse if it is only related to the concept ”Algebra” since the other aspects about the examinee are missing.
In one word, we propose two goals for the strategy in MAAT framework:
(1) \textbf{quality}: to select informative questions containing as much information as possible;
(2) \textbf{diversity}: to cover as many knowledge concepts as possible in the selected question set.

% 介绍我们的框架实现细节
We implement our MAAT framework with three cooperating modules,
which selects one question that optimizes both quality and diversity at each step consisting of two stages.
At the first stage, we select a small candidate subset of the most high-quality questions in Quality Module, which quantifies the quality of questions with a model-agnostic function named Expected Model Change (EMC).
At the second stage, we select one question from the candidate subset in Diversity Module, which efficiently optimizes the diversity of the selected questions by the marginal gain of the Importance Weighted Knowledge Coverage (IWKC).
In addition, we make full use of the historical data to pre-compute the importance weight of each knowledge concept in Importance Module.

% 实验
Finally, we conduct extensive experiments on two real-world educational datasets.
The experimental results show that the proposed MAAT framework can effectively optimize both informativeness and diversity in a model-agnostic way.
It is worth noting that CAT is appliable to many other scenarios besides education, such as vocation and psychology, etc.



